The azimuthal correlation between the leading jet and the scattered lepton in deep inelastic scattering at HERA

The azimuthal correlation angle, $\Delta\phi$, between the scattered lepton and the leading jet in deep inelastic $e^{\pm}p$ scattering at HERA has been studied using data collected with the ZEUS detector at a centre-of-mass energy of $\sqrt{s} = 318 \;\mathrm{GeV}$, corresponding to an integrated luminosity of $326 \;\mathrm{pb}^{-1}$. A measurement of jet cross sections in the laboratory frame was made in a fiducial region corresponding to photon virtuality $10 \;\mathrm{GeV}^2 < Q^2 < 350 \;\mathrm{GeV}^2$, inelasticity $0.04 < y < 0.7$, outgoing lepton energy $E_e > 10 \;\mathrm{GeV}$, lepton polar angle $140^\circ < \theta_e < 180^\circ$, jet transverse momentum $2.5 \;\mathrm{GeV} < p_\mathrm{T,jet} < 30 \;\mathrm{GeV}$, and jet pseudorapidity $-1.5 < \eta_\mathrm{jet} < 1.8$. Jets were reconstructed using the $k_\mathrm{T}$ algorithm with the radius parameter $R = 1$. The leading jet in an event is defined as the jet that carries the highest $p_\mathrm{T,jet}$. Differential cross sections, $d\sigma/d\Delta\phi$, were measured as a function of the azimuthal correlation angle in various ranges of leading-jet transverse momentum, photon virtuality and jet multiplicity. Perturbative calculations at $\mathcal{O}(\alpha_{s}^2)$ accuracy successfully describe the data within the fiducial region, although a lower level of agreement is observed near $\Delta\phi \rightarrow \pi$ for events with high jet multiplicity, due to limitations of the perturbative approach in describing soft phenomena in QCD. The data are equally well described by Monte Carlo predictions that supplement leading-order matrix elements with parton showering.

==> LaTeX/examples/Kconf/zconf-tit.tex <==
\titlehead{\centering
Submitted to the\\\textbf{XXX$^{\rm th}$
International Conference on High Energy Physics\\Osaka, Japan,
July 27 -- August 2, 2000}
\vspace*{3mm}
\hrule
\vspace*{3mm}
\parbox[t]{5cm}{Abstract: 9999}%
\hfill%
\parbox[t]{5cm}{\raggedleft
Plenary Session: M\\Parallel Session: K}
}

% If your abstract is very long reduce \zeustitlespace a bit
% \addtolength{\zeustitlespace}{-0.5cm}
\zeustitle{%
  Search for a Better Life in Deep Inelastic
  $\mathbf{e^+p \to e^+X}$ Scattering at HERA
}

\zeusauthor{ZEUS Collaboration}
\draftversion{0.1}
% Set \zeusdate to empty for final preprint.
% \zeusdate{}
% \zeusdate{27 May 2011}

\maketitle

% If you use the package siunitx instead of units you have to change
% \unit to \SI, to enclose the values in curly brackets and change
% \pbi to \per\pb and \Gev to \GeV, e.g. \SI{47.7}{\per\pb}
%
% If you use the package hepunits instead of units you have to enclose
% the values in curly brackets and change \pbi to \invpb and \Gev to \GeV
% e.g. \unit{47.7}{\invpb}
% If the quantity is not in math mode and the unit contains math mode
% characters such as superscripts it must be contained in $...$
%
\begin{abstract}\noindent
  In a search for a better life beyond the Standard Model, various
  hypotheses have been tested using the high-$Q^2$, deep inelastic
  neutral current $e^+p$ scattering data collected with the ZEUS
  detector at HERA.  The data correspond to an integrated luminosity
  of $\unit[47.7]{\pbi}$ of $e^+p$ interactions at \unit[300]{\Gev}
  centre-of-mass energy. No significant evidence for holidays has been
  found.  Lower limits at the \unit[95]{\%} confidence level are set on the
  average monthly working time of a physicist.
\end{abstract}


==> LaTeX/examples/Kconf/zconf-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots At some
place you might in particular like to introduce the CTD \citeCTD, the
MVD \citeMVD and the ZEUS calorimeter \citeCAL.

\clearpage


==> LaTeX/examples/Kdraft/zdraft-tit.tex <==
% These are needed when draft mode is changed to preprint mode
% \prepnum{DESY--13--NNN}
% \prepdate{MMMM 2013}

% If your abstract is very long reduce \zeustitlespace a bit
% \addtolength{\zeustitlespace}{-0.5cm}
\zeustitle{%
  Search for a Better Life in Deep Inelastic
  $\mathbf{e^+p \to e^+X}$ Scattering at HERA
}

\zeusauthor{ZEUS Collaboration}
\draftversion{0.1}
% Set \zeusdate to empty for final preprint.
% \zeusdate{}
% \zeusdate{27 May 2011}

\maketitle

% If you use the package siunitx instead of units you have to change
% \unit to \SI, to enclose the values in curly brackets and change
% \pbi to \per\pb and \Gev to \GeV, e.g. \SI{47.7}{\per\pb}
%
% If you use the package hepunits instead of units you have to enclose
% the values in curly brackets and change \pbi to \invpb and \Gev to \GeV
% e.g. \unit{47.7}{\invpb}
% If the quantity is not in math mode and the unit contains math mode
% characters such as superscripts it must be contained in $...$
%
\begin{abstract}\noindent
  In a search for a better life beyond the Standard Model, various
  hypotheses have been tested using the high-$Q^2$, deep inelastic
  neutral current $e^+p$ scattering data collected with the ZEUS
  detector at HERA.  The data correspond to an integrated luminosity
  of $\unit[47.7]{\pbi}$ of $e^+p$ interactions at \unit[300]{\Gev}
  centre-of-mass energy. No significant evidence for holidays has been
  found.  Lower limits at the \unit[95]{\%} confidence level are set on the
  average monthly working time of a physicist.
\end{abstract}


==> LaTeX/examples/Kdraft/zdraft-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your introductory text.

% ----------------------------------------------------------------------------
%       Experimental set-up
% ----------------------------------------------------------------------------
\section{Experimental set-up}
\label{sec-exp}

Here you might want to describe your data samples and the detctor. In
particular, you may use some of the text fragments provided as \LaTeXZ
macros. These can all be found in the file
\texttt{LaTeX/zeus/zeusdet\_units.tex},
\texttt{LaTeX/zeus/zeusdet\_hepunits.tex} or
\texttt{LaTeX/zeus/zeusdet\_siunitx.tex} depending on whether you use the
\texttt{units} (default), \texttt{hepunits} or \texttt{siunitx}
package for typesetting units.

% ----------------------------------------------------------------------------
%       General detector blabla
% ----------------------------------------------------------------------------
\Zdetdesc

% ----------------------------------------------------------------------------
%       CTD+MVD description, footnote on coordinate system is the argument
% ----------------------------------------------------------------------------
\Zctdmvddesc{\ZcoosysfnBEeta}

% ----------------------------------------------------------------------------
%       CAL description straight and simple
% ----------------------------------------------------------------------------
\Zcaldesc

% ----------------------------------------------------------------------------
%       Muon system description. You may want it or not. No references for it
% ----------------------------------------------------------------------------
\Zmuondesc

% ----------------------------------------------------------------------------
%       BAC description complete with reference
% ----------------------------------------------------------------------------
\Zbacdesc

% ----------------------------------------------------------------------------
%       LUMI, give actual luminosity uncertainty in % for your sample as argument
%       Use \Zlumidesc is you don't want the uncertainty here.
% ----------------------------------------------------------------------------
\ZlumidescA{2.6}

\clearpage


% ----------------------------------------------------------------------------
%       Mandatory acknowledgements. You may add your buddies to it.
% ----------------------------------------------------------------------------
\section*{Acknowledgements}
\label{sec-ack}

\Zacknowledge

\clearpage


==> LaTeX/examples/Knote/znote-tit.tex <==
\prepnum{ZEUS--13--NNN}
\prepdate{\today}

% If your abstract is very long reduce \zeustitlespace a bit
% \addtolength{\zeustitlespace}{-0.5cm}
\zeustitle{%
  Calibration of the Mood of the Operators\\
  in the ZEUS Running 2006/2007
}

\zeusauthor{Your name\\
        {\small\it your email}\\[3.mm]
        {\large Your institution}\\
        {\large \it address}
}
% \zeusdate{27 May 2011}

\maketitle

\begin{abstract}\noindent
  In previous years, strong dependences of data taking efficiencies
  and physics results on the mood of the ZEUS shift crew have been
  observed.  We report on an attempt to automatically monitor and
  adjust the relevant parameters by supplying moderate doses of
  beer. It can be shown that this approach stabilizes the
  situation. However, remaining dependences, in particular on the moon
  phase, are still to be corrected for.
\end{abstract}


==> LaTeX/examples/Knote/znote-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots At some
place you might in particular like to introduce the CTD \citeCTD, the
MVD \citeMVD and the ZEUS calorimeter \citeCAL.
\vfill\eject


==> LaTeX/examples/Kother/zother-ref.tex <==
{
% \def\bibname{\Large\bf References}
% \def\refname{\Large\bf References}
% \pagestyle{plain}
%
%  If you (have to) use a different bibliography style file than
%  l4z_default.bst (or one of its clones derived from zeusbtxbst.bdc),
%  you will have to apply several adjustments to it:
%  - Add the fields "checked", "eprint", "replaces" and "replacedby",
%    "report", "submitdate" and "www" to the ENTRY section.
%  - Add a appropriate definitions for entry types "Preprint" and
%    "Thesis".
%
%  You will probably decide that it is horribly complicated to get
%  this working.
%  I offer support for two types of possible solutions:
%  (i)  try to adhere to the required standards by choosing the
%       appropriate flags in zeusbtxbst.bdc and adapting the
%       resulting bst file as necessary
%  (ii) take the bst file provided by the editor or publishing
%       institution and adapt it to the data fields and conventions
%       in the LaTeX4zeus bibligraphy database.
%
%  I cannot promise that either of both possibilities works, but
%  in general there should be a solution which allows to use the
%  LaTeX4zeus bibligraphy database. Please contact me (Ian Brock,
%  brock@physik.uni-bonn.de) for further support.
%
%  Please report technical problems using the LaTeX4zeus message form:
%  http://www-zeus.desy.de/ZEUS_ONLY/LaTeX4zeus/WWW/php/l4z_message.php3
%
\bibliographystyle{./BiBTeX/bst/l4z_default3}
{\raggedright
% Comma-separated list of bib files
\bibliography{./BiBTeX/bib/l4z_zeus.bib}}
}
\vfill\eject


==> LaTeX/examples/Kother/zother-tit.tex <==
%
%  Title page and abstract.
%  ------------------------
%  Note that the abstract is not included in the standard title page
%  of article.cls (and therefore appears on a separate page). Other
%  class files may define additional or different elements of the title
%  page.
%

\title{%
  A Scientific Report\\
  Typeset in the \LaTeXZ Environment\\
  Without Using \texttt{zeus{\usc}paper.cls}
}

\author{Your name\\
        {\small\it your email}\\[3.mm]
        Your institution\\
        {\it address}\\
}
% \date{27 May 2011}

\maketitle

\begin{abstract}\noindent
  The \LaTeXZ environment provides access to a large bibliography
  data base and a set of utility macros which can be used also outside
  the framework set up in the \LaTeX{} class file \texttt{zeus{\usc}paper.cls}.
  This report may serve as an example.
\end{abstract}

==> LaTeX/examples/Kother/zother-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots

At some place you might in particular like to introduce the CTD
\citeCTD, the MVD \citeMVD and the ZEUS calorimeter \citeCAL. If not,
these references may serve as examples for the use of definitions in
\texttt{zother-cit.tex}.

\vfill\eject


==> LaTeX/examples/Kprep/zprep-tit.tex <==
% These are needed when draft mode is changed to preprint mode
\prepnum{DESY--13--NNN}
\prepdate{MMMM 2013}

% If your abstract is very long reduce \zeustitlespace a bit
% \addtolength{\zeustitlespace}{-0.5cm}
\zeustitle{%
  Search for a Better Life in Deep Inelastic
  $\mathbf{e^+p \to e^+X}$ Scattering at HERA
}

\zeusauthor{ZEUS Collaboration}
% Set \zeusdate to empty for final preprint.
\zeusdate{}
% \zeusdate{27 May 2011}

\maketitle

% If you use the package siunitx instead of units you have to change
% \unit to \SI, to enclose the values in curly brackets and change
% \pbi to \per\pb and \Gev to \GeV, e.g. \SI{47.7}{\per\pb}
%
% If you use the package hepunits instead of units you have to enclose
% the values in curly brackets and change \pbi to \invpb and \Gev to \GeV
% e.g. \unit{47.7}{\invpb}
% If the quantity is not in math mode and the unit contains math mode
% characters such as superscripts it must be contained in $...$
%
\begin{abstract}\noindent
  In a search for a better life beyond the Standard Model, various
  hypotheses have been tested using the high-$Q^2$, deep inelastic
  neutral current $e^+p$ scattering data collected with the ZEUS
  detector at HERA.  The data correspond to an integrated luminosity
  of $\unit[47.7]{\pbi}$ of $e^+p$ interactions at \unit[300]{\Gev}
  centre-of-mass energy. No significant evidence for holidays has been
  found.  Lower limits at the \unit[95]{\%} confidence level are set on the
  average monthly working time of a physicist.
\end{abstract}


==> LaTeX/examples/Kprep/zprep-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your introductory text.

% ----------------------------------------------------------------------------
%       Experimental set-up
% ----------------------------------------------------------------------------
\section{Experimental set-up}
\label{sec-exp}

Here you might want to describe your data samples and the detctor. In
particular, you may use some of the text fragments provided as \LaTeXZ
macros. These can all be found in the file
\texttt{LaTeX/zeus/zeusdet\_units.tex},
\texttt{LaTeX/zeus/zeusdet\_hepunits.tex} or
\texttt{LaTeX/zeus/zeusdet\_siunitx.tex} depending on whether you use the
\texttt{units} (default), \texttt{hepunits} or \texttt{siunitx}
package for typesetting units.

% ----------------------------------------------------------------------------
%       General detector blabla
% ----------------------------------------------------------------------------
\Zdetdesc

% ----------------------------------------------------------------------------
%       CTD+MVD description, footnote on coordinate system is the argument
% ----------------------------------------------------------------------------
\Zctdmvddesc{\ZcoosysfnBEeta}

% ----------------------------------------------------------------------------
%       CAL description straight and simple
% ----------------------------------------------------------------------------
\Zcaldesc

% ----------------------------------------------------------------------------
%       Muon system description. You may want it or not. No references for it
% ----------------------------------------------------------------------------
\Zmuondesc

% ----------------------------------------------------------------------------
%       BAC description complete with reference
% ----------------------------------------------------------------------------
\Zbacdesc

% ----------------------------------------------------------------------------
%       LUMI, give actual luminosity uncertainty in % for your sample as argument
%       Use \Zlumidesc is you don't want the uncertainty here.
% ----------------------------------------------------------------------------
\ZlumidescA{2.6}

\clearpage


% ----------------------------------------------------------------------------
%       Mandatory acknowledgements. You may add your buddies to it.
% ----------------------------------------------------------------------------
\section*{Acknowledgements}
\label{sec-ack}

\Zacknowledge

\clearpage


==> LaTeX/examples/common/zcommon-aut.tex <==
%=================================================================== 
%
%  This file will be replaced with the "official" author
%  list which is created for each ZEUS paper individually.
%
%===================================================================== 
\pagenumbering{Roman} 

\begin{center} 
{\Large  The ZOOPS Collaboration}
\end{center}

{\raggedright
  F.~Author$^{1}$,
  A.~Nother,
  X.~Whoever\\
 {\it Absolutely Non-Existing Institute of Nothing, Nowhere, Country}~$^{a}$ 
}

\par\filbreak
\begin{supertabular}[h]{rp{14cm}}
$^{\ 1}$ & now visiting a scientist next door\\ 
\end{supertabular}

\begin{tabular}[h]{rp{14cm}}
$^{a}$ &  supported by the National Council of Nonsense (NCNS)\\ 
\end{tabular} 


==> LaTeX/examples/common/zcommon-cit.tex <==
%==============================================================================
% Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
% -> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,*npps:b32:181,*nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
% -> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
% -> STT
%------------------------------------------------------------------------------
\def\citeSTT{{\cite{%
nim:a535:191%
}}\xspace}
%------------------------------------------------------------------------------
% -> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,*nim:a309:101,*nim:a321:356,*nim:a336:23%
}}\xspace}
%------------------------------------------------------------------------------
% -> HES
%------------------------------------------------------------------------------
\def\citeHES{{\cite{%
nim:a277:176%
}}\xspace}
%------------------------------------------------------------------------------
% -> 6mT
%------------------------------------------------------------------------------
\def\citeSixmT{{\cite{%
thesis:gosau:2007%
}}\xspace}
%------------------------------------------------------------------------------
% -> BAC
%------------------------------------------------------------------------------
\def\citeBAC{{\cite{%
nim:a300:480%
}}\xspace}
%------------------------------------------------------------------------------
% -> LUMI
%------------------------------------------------------------------------------
\def\citePCAL{{\cite{%
desy-92-066,*zfp:c63:391,*acpp:b32:2025%
}}\xspace}
\def\citeSPECTRO{{\cite{%
nim:a565:572%
}}\xspace}


==> LaTeX/examples/common/zcommon-cit_nomcite.tex <==
%==============================================================================
% Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
% -> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,npps:b32:181,nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
% -> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
% -> STT
%------------------------------------------------------------------------------
\def\citeSTT{{\cite{%
nim:a535:191%
}}\xspace}
%------------------------------------------------------------------------------
% -> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,nim:a309:101,nim:a321:356,nim:a336:23%
}}\xspace}
%------------------------------------------------------------------------------
% -> HES
%------------------------------------------------------------------------------
\def\citeHES{{\cite{%
nim:a277:176%
}}\xspace}
%------------------------------------------------------------------------------
% -> 6mT
%------------------------------------------------------------------------------
\def\citeSixmT{{\cite{%
thesis:gosau:2007%
}}\xspace}
%------------------------------------------------------------------------------
% -> BAC
%------------------------------------------------------------------------------
\def\citeBAC{{\cite{%
nim:a300:480%
}}\xspace}
%------------------------------------------------------------------------------
% -> LUMI
%------------------------------------------------------------------------------
\def\citePCAL{{\cite{%
desy-92-066,zfp:c63:391,acpp:b32:2025%
}}\xspace}
\def\citeSPECTRO{{\cite{%
nim:a565:572%
}}\xspace}


==> LaTeX/examples/common/zcommon-fig.tex <==
%-------------------------------------------------------------------------------
%       Results
%-------------------------------------------------------------------------------
\begin{figure}[p]
\vfill
\begin{center}
\framebox[13.cm]{\rule{0.pt}{10.cm}}
\end{center}
\caption{
Life beyond the Standard Model.}
\label{fig-contfey}
\vfill
\end{figure}


==> LaTeX/examples/common/zcommon-ref.tex <==
{
% \def\bibname{\normalfont\Large\bfseries References}
% \def\refname{\normalfont\Large\bfseries References}
% \pagestyle{plain}
\ifzeusbst
  \ifzmcite
     \bibliographystyle{./BiBTeX/bst/l4z_default3}
  \else
     \bibliographystyle{./BiBTeX/bst/l4z_default3_nomcite}
  \fi
\fi
\ifzdrftbst
  \ifzmcite
    \bibliographystyle{./BiBTeX/bst/l4z_draft3}
  \else
    \bibliographystyle{./BiBTeX/bst/l4z_draft3_nomcite}
  \fi
\fi
\ifzbstepj
  \ifzmcite
    \bibliographystyle{./BiBTeX/bst/l4z_epj3}
  \else
    \bibliographystyle{./BiBTeX/bst/l4z_epj3_nomcite}
  \fi
\fi
\ifzbstjhep
  \ifzmcite
    \bibliographystyle{./BiBTeX/bst/l4z_jhep3}
  \else
    \bibliographystyle{./BiBTeX/bst/l4z_jhep3_nomcite}
  \fi
\fi
\ifzbstnp
  \ifzmcite
    \bibliographystyle{./BiBTeX/bst/l4z_np3}
  \else
    \bibliographystyle{./BiBTeX/bst/l4z_np3_nomcite}
  \fi
\fi
\ifzbstpl
  \ifzmcite
    \bibliographystyle{./BiBTeX/bst/l4z_pl3}
  \else
    \bibliographystyle{./BiBTeX/bst/l4z_pl3_nomcite}
  \fi
\fi
{\raggedright
\bibliography{./syn.bib,%
              ./myref.bib,%
              ./BiBTeX/bib/l4z_zeus.bib,%
              ./BiBTeX/bib/l4z_h1.bib,%
              ./BiBTeX/bib/l4z_articles.bib,%
              ./BiBTeX/bib/l4z_books.bib,%
              ./BiBTeX/bib/l4z_conferences.bib,%
              ./BiBTeX/bib/l4z_misc.bib,%
              ./BiBTeX/bib/l4z_preprints.bib}}
}
\vfill\eject


==> LaTeX/examples/common/zcommon-tab.tex <==
%-------------------------------------------------------------------------------
%       An example table
%-------------------------------------------------------------------------------
\begin{table}[p]
\begin{center}
\begin{tabular}{||c|rrrr|rrrr||}
\hline
Label & $\eta^u_{LL}$ & $\eta^u_{LR}$ & $\eta^u_{RL}$ & $\eta^u_{RR}$ & 
        $\eta^d_{LL}$ & $\eta^d_{LR}$ & $\eta^d_{RL}$ & $\eta^d_{RR}$ \\ 
\hline\hline
VV&  $+1$&$+1$&$+1$&$+1$&
     $+1$&$+1$&$+1$&$+1$ \\
AA&  $+1$&$-1$&$-1$&$+1$&
     $+1$&$-1$&$-1$&$+1$ \\
VA&  $+1$&$-1$&$+1$&$-1$&
     $+1$&$-1$&$+1$&$-1$ \\
X1&  $+1$&$-1$&$ 0$&$ 0$&
     $+1$&$-1$&$ 0$&$ 0$ \\
X2&  $+1$&$ 0$&$+1$&$ 0$&
     $+1$&$ 0$&$+1$&$ 0$ \\
X3&  $+1$&$ 0$&$ 0$&$+1$&
     $+1$&$ 0$&$ 0$&$+1$ \\
X4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$+1$&$+1$&$ 0$ \\
X5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$+1$&$ 0$&$+1$ \\
X6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$+1$&$-1$ \\
U1&  $+1$&$-1$&$ 0$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U2&  $+1$&$ 0$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U3&  $+1$&$ 0$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
\hline
\end{tabular}
\caption{The 30 scenarios for a better life considered in this paper.
         Each row of this table corresponds to two different scenarios for
         overall interference signs $\epsilon=+1$ and $\epsilon=-1$, 
         respectively.}
  \label{tab-models}
\end{center}
\end{table}


==> LaTeX/examples/conf/zconf-tit.tex <==
\prepnum{DESY--13--NNN}

\title{%
Search for a Better Life
in Deep Inelastic $\mathbf{e^+p\to e^+X}$ Scattering
at HERA
}

\author{ZEUS Collaboration}
\draftversion{0.1}
% \date{27 May 2011}

\confname{XXX$^{\rm th}$ International Conference on High Energy Physics}
\confplacedate{Osaka, Japan, July 27 -- August 2, 2000}
\confsession{Plenary Session: M\\Parallel Session: K}
\confabsnum{9999}

% If you use the package siunitx instead of units you have to change
% \unit to \SI, to enclose the values in curly brackets and change
% \pbi to \per\pb and \Gev to \GeV, e.g. \SI{47.7}{\per\pb}
%
% If you use the package hepunits instead of units you have to enclose
% the values in curly brackets and change \pbi to \invpb and \Gev to \GeV
% e.g. \unit{47.7}{\invpb}
% If the quantity is not in math mode and the unit contains math mode
% characters such as superscripts it must be contained in $...$
%
\abstract{%
  In a search for a better life beyond the Standard Model, various
  hypotheses have been tested using the high-$Q^2$, deep inelastic
  neutral current $e^+p$ scattering data collected with the ZEUS
  detector at HERA.  The data correspond to an integrated luminosity
  of $\unit[47.7]{\pbi}$ of $e^+p$ interactions at \unit[300]{\Gev}
  centre-of-mass energy. No significant evidence for holidays has been
  found.  Lower limits at the \unit[95]{\%} confidence level are set on the
  average monthly working time of a physicist.
}

\makezeustitle


==> LaTeX/examples/conf/zconf-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots At some
place you might in particular like to introduce the CTD \citeCTD, the
MVD \citeMVD and the ZEUS calorimeter \citeCAL.

\clearpage


==> LaTeX/examples/draft/zdraft-tit.tex <==
% This is needed when draft mode is changed to preprint mode
\prepnum{DESY--13--NNN}

\title{%
Search for a Better Life
in Deep Inelastic $\mathbf{e^+p\to e^+X}$ Scattering
at HERA
}

\author{ZEUS Collaboration}
\draftversion{0.1}
% Set \date for final preprint.
% \date{MMMM 2013}
% \date{27 May 2011}

% If you use the package siunitx instead of units you have to change
% \unit to \SI, to enclose the values in curly brackets and change
% \pbi to \per\pb and \Gev to \GeV, e.g. \SI{47.7}{\per\pb}
%
% If you use the package hepunits instead of units you have to enclose
% the values in curly brackets and change \pbi to \invpb and \Gev to \GeV
% e.g. \unit{47.7}{\invpb}
% If the quantity is not in math mode and the unit contains math mode
% characters such as superscripts it must be contained in $...$
%
\abstract{%
  In a search for a better life beyond the Standard Model, various
  hypotheses have been tested using the high-$Q^2$, deep inelastic
  neutral current $e^+p$ scattering data collected with the ZEUS
  detector at HERA.  The data correspond to an integrated luminosity
  of $\unit[47.7]{\pbi}$ of $e^+p$ interactions at \unit[300]{\Gev}
  centre-of-mass energy. No significant evidence for holidays has been
  found.  Lower limits at the \unit[95]{\%} confidence level are set on the
  average monthly working time of a physicist.
}

\makezeustitle


==> LaTeX/examples/draft/zdraft-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your introductory text.

% ----------------------------------------------------------------------------
%       Experimental set-up
% ----------------------------------------------------------------------------
\section{Experimental set-up}
\label{sec-exp}

Here you might want to describe your data samples and the detctor. In
particular, you may use some of the text fragments provided as \LaTeXZ
macros. These can all be found in the file
\texttt{LaTeX/zeus/zeusdet\_units.tex},
\texttt{LaTeX/zeus/zeusdet\_hepunits.tex} or
\texttt{LaTeX/zeus/zeusdet\_siunitx.tex} depending on whether you use the
\texttt{units} (default), \texttt{hepunits} or \texttt{siunitx}
package for typesetting units.

% ----------------------------------------------------------------------------
%       General detector blabla
% ----------------------------------------------------------------------------
\Zdetdesc

% ----------------------------------------------------------------------------
%       CTD+MVD description, footnote on coordinate system is the argument
% ----------------------------------------------------------------------------
\Zctdmvddesc{\ZcoosysfnBEeta}

% ----------------------------------------------------------------------------
%       CAL description straight and simple
% ----------------------------------------------------------------------------
\Zcaldesc

% ----------------------------------------------------------------------------
%       Muon system description. You may want it or not. No references for it
% ----------------------------------------------------------------------------
\Zmuondesc

% ----------------------------------------------------------------------------
%       BAC description complete with reference
% ----------------------------------------------------------------------------
\Zbacdesc

% ----------------------------------------------------------------------------
%       LUMI, give actual luminosity uncertainty in % for your sample as argument
%       Use \Zlumidesc is you don't want the uncertainty here.
% ----------------------------------------------------------------------------
\ZlumidescA{2.6}

\clearpage


% ----------------------------------------------------------------------------
%       Mandatory acknowledgements. You may add your buddies to it.
% ----------------------------------------------------------------------------
\section*{Acknowledgements}
\label{sec-ack}

\Zacknowledge

\clearpage


==> LaTeX/examples/note/znote-tit.tex <==
\prepnum{ZEUS--13--NNN}

\title{
Calibration of the Mood of the Operators\\
in the ZEUS Running 2006/2007
}

\author{Your name\\
        {\small\it your email}\\[3.mm]
        {\large Your institution}\\
        {\large \it address}
}
% \date{27 May 2011}

\abstract{%
  In previous years, strong dependences of data taking efficiencies
  and physics results on the mood of the ZEUS shift crew have been
  observed.  We report on an attempt to automatically monitor and
  adjust the relevant parameters by supplying moderate doses of
  beer. It can be shown that this approach stabilizes the
  situation. However, remaining dependences, in particular on the moon
  phase, are still to be corrected for.
}

\makezeustitle


==> LaTeX/examples/note/znote-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots At some
place you might in particular like to introduce the CTD \citeCTD, the
MVD \citeMVD and the ZEUS calorimeter \citeCAL.
\vfill\eject


==> LaTeX/examples/other/zother-ref.tex <==
{
% \def\bibname{\Large\bf References}
% \def\refname{\Large\bf References}
% \pagestyle{plain}
%
%  If you (have to) use a different bibliography style file than
%  l4z_default.bst (or one of its clones derived from zeusbtxbst.bdc),
%  you will have to apply several adjustments to it:
%  - Add the fields "checked", "eprint", "replaces" and "replacedby",
%    "report", "submitdate" and "www" to the ENTRY section.
%  - Add a appropriate definitions for entry types "Preprint" and
%    "Thesis".
%
%  You will probably decide that it is horribly complicated to get
%  this working.
%  I offer support for two types of possible solutions:
%  (i)  try to adhere to the required standards by choosing the
%       appropriate flags in zeusbtxbst.bdc and adapting the
%       resulting bst file as necessary
%  (ii) take the bst file provided by the editor or publishing
%       institution and adapt it to the data fields and conventions
%       in the LaTeX4zeus bibligraphy database.
%
%  I cannot promise that either of both possibilities works, but
%  in general there should be a solution which allows to use the
%  LaTeX4zeus bibligraphy database. Please contact me (Ian Brock,
%  brock@physik.uni-bonn.de) for further support.
%
%  Please report technical problems using the LaTeX4zeus message form:
%  http://www-zeus.desy.de/ZEUS_ONLY/LaTeX4zeus/WWW/php/l4z_message.php3
%
\bibliographystyle{./BiBTeX/bst/l4z_default3}
{\raggedright
% Comma-separated list of bib files
\bibliography{./BiBTeX/bib/l4z_zeus.bib}}
}
\vfill\eject


==> LaTeX/examples/other/zother-tit.tex <==
%
%  Title page and abstract.
%  ------------------------
%  Note that the abstract is not included in the standard title page
%  of article.cls (and therefore appears on a separate page). Other
%  class files may define additional or different elements of the title
%  page.
%

\title{
A Scientific Report\\
Typeset in the \LaTeXZ Environment\\
Without Using \texttt{zeus{\usc}paper.cls}
}

\author{Your name\\
        {\small\it your email}\\[3.mm]
        Your institution\\
        {\it address}\\
}
% \date{27 May 2011}

\maketitle

\noindent{\bf Abstract:}
The \LaTeXZ environment provides access to a large bibliography
data base and a set of utility macros which can be used also outside
the framework set up in the \LaTeX{} class file \texttt{zeus{\usc}paper.cls}.
This report may serve as an example.


==> LaTeX/examples/other/zother-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots

At some place you might in particular like to introduce the CTD
\citeCTD, the MVD \citeMVD and the ZEUS calorimeter \citeCAL. If not,
these references may serve as examples for the use of definitions in
\texttt{zother-cit.tex}.

\vfill\eject


==> LaTeX/examples/prep/zprep-tit.tex <==
% This is needed when draft mode is changed to preprint mode
\prepnum{DESY--13--NNN}

\title{%
Search for a Better Life
in Deep Inelastic $\mathbf{e^+p\to e^+X}$ Scattering
at HERA
}

\author{ZEUS Collaboration}
% Set \date for final preprint.
\date{MMMM 2013}
% \date{27 May 2011}

% If you use the package siunitx instead of units you have to change
% \unit to \SI, to enclose the values in curly brackets and change
% \pbi to \per\pb and \Gev to \GeV, e.g. \SI{47.7}{\per\pb}
%
% If you use the package hepunits instead of units you have to enclose
% the values in curly brackets and change \pbi to \invpb and \Gev to \GeV
% e.g. \unit{47.7}{\invpb}
% If the quantity is not in math mode and the unit contains math mode
% characters such as superscripts it must be contained in $...$
%
\abstract{%
  In a search for a better life beyond the Standard Model, various
  hypotheses have been tested using the high-$Q^2$, deep inelastic
  neutral current $e^+p$ scattering data collected with the ZEUS
  detector at HERA.  The data correspond to an integrated luminosity
  of $\unit[47.7]{\pbi}$ of $e^+p$ interactions at \unit[300]{\Gev}
  centre-of-mass energy. No significant evidence for holidays has been
  found.  Lower limits at the \unit[95]{\%} confidence level are set on the
  average monthly working time of a physicist.
}

\makezeustitle


==> LaTeX/examples/prep/zprep-txt.tex <==
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your introductory text.

% ----------------------------------------------------------------------------
%       Experimental set-up
% ----------------------------------------------------------------------------
\section{Experimental set-up}
\label{sec-exp}

Here you might want to describe your data samples and the detctor. In
particular, you may use some of the text fragments provided as \LaTeXZ
macros. These can all be found in the file
\texttt{LaTeX/zeus/zeusdet\_units.tex},
\texttt{LaTeX/zeus/zeusdet\_hepunits.tex} or
\texttt{LaTeX/zeus/zeusdet\_siunitx.tex} depending on whether you use the
\texttt{units} (default), \texttt{hepunits} or \texttt{siunitx}
package for typesetting units.

% ----------------------------------------------------------------------------
%       General detector blabla
% ----------------------------------------------------------------------------
\Zdetdesc

% ----------------------------------------------------------------------------
%       CTD+MVD description, footnote on coordinate system is the argument
% ----------------------------------------------------------------------------
\Zctdmvddesc{\ZcoosysfnBEeta}

% ----------------------------------------------------------------------------
%       CAL description straight and simple
% ----------------------------------------------------------------------------
\Zcaldesc

% ----------------------------------------------------------------------------
%       Muon system description. You may want it or not. No references for it
% ----------------------------------------------------------------------------
\Zmuondesc

% ----------------------------------------------------------------------------
%       BAC description complete with reference
% ----------------------------------------------------------------------------
\Zbacdesc

% ----------------------------------------------------------------------------
%       LUMI, give actual luminosity uncertainty in % for your sample as argument
%       Use \Zlumidesc is you don't want the uncertainty here.
% ----------------------------------------------------------------------------
\ZlumidescA{2.6}

\clearpage


% ----------------------------------------------------------------------------
%       Mandatory acknowledgements. You may add your buddies to it.
% ----------------------------------------------------------------------------
\section*{Acknowledgements}
\label{sec-ack}

\Zacknowledge

\clearpage


==> LaTeX/examples/talk/ztalk-fmt.tex <==
%------------------------------------------------------------------------------
%       interline spacing, paragraph indention etc.
%------------------------------------------------------------------------------
\renewcommand{\baselinestretch}{1.0}
\renewcommand{\arraystretch}{1.1}
\parindent       0.0pt
\parskip         3.5pt
\overfullrule    0.0pt
%------------------------------------------------------------------------------
%       item spacings
%------------------------------------------------------------------------------
\itemsep    0.2ex plus 0.1ex minus 0.15ex
\topsep     0.2ex plus 0.1ex minus 0.15ex
\partopsep  0.2ex plus 0.1ex minus 0.1ex
\setlength\leftmargini   {1.6em}
\setlength\leftmarginii  {1.2em}
\setlength\leftmarginiii {1.0em}
\setlength\leftmarginiv  {0.8em}
%------------------------------------------------------------------------------
%       define colored bullet with distance for pseudo-itemize environment
%------------------------------------------------------------------------------
\def\cbullet#1{{#1\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern1.em}
\def\cbull#1#2{{#1\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern#2}
\def\carrow#1{{#1$\mbs{\to}$}\kern0.55em}
\def\cminus#1{{\bf#1--}\kern0.8em}
\def\cmin#1#2{{\bf#1--}\kern#2}
\def\cplus#1{{#1$\mbs{+}$}\kern0.8em}
\def\cplu#1#2{{#1$\mbs{+}$}\kern#2}
\def\cequal#1{{#1$\mbs{=}$}\kern0.7em}
\def\csurd#1{{#1$\mbs{\surd}$}\kern1.em}
\def\csur#1#2{{#1$\mbs{\surd}$}\kern#2}
\def\pbullet{\phantom{{\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern1.em}}
\def\pbull#1{\phantom{{\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern#1}}
\def\parrow{\phantom{{$\mbs{\to}$}\kern0.55em} }
\def\pminus{\phantom{{\bf--}\kern0.8em} }
\def\pequal{\phantom{{$\mbs{=}$}\kern0.7em} }
\def\psurd{\phantom{{$\mbs{\surd}$}\kern1.em} }
\def\psur#1{\phantom{{$\mbs{\surd}$}\kern#1} }
%------------------------------------------------------------------------------
%       "tight item" environment
%------------------------------------------------------------------------------
\newenvironment{tightitemize}[2]
 {\begin{list}{$\bullet$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
%------------------------------------------------------------------------------
%       Define mathbfs
%       --------------
%------------------------------------------------------------------------------
\DeclareMathAlphabet{\mathbfs}{OT1}{lcmss}{bx}{sl}
%\DeclareMathAlphabet{\mathbfs}{OT1}{cmr}{bx}{sl}
\def\mbs{\mathbfs}
%------------------------------------------------------------------------------
%       boxpage decoration
%       ------------------
%------------------------------------------------------------------------------
\newcounter{chap}
\newcounter{chapslide}
\setcounter{chapslide}{0}
\renewcommand{\footerleft}{U.~Katz}
\renewcommand{\footerright}{\thechap.\thechapslide}
\renewcommand{\footercenter}{\LaTeXZ}
\renewcommand{\bpdtcolor}{money}
\renewcommand{\bpdtype}{B}
\renewcommand{\boxpagedecoration}{%
  \strut\kern-1.7cm
  \begin{turn}{90}
    \begin{minipage}{\textheight}
      \begin{center}
        \color{darkred}
        {\tiny{\usefont{OT1}{cmr}{m}{sc}
               ZEUS Collaboration Meeting, 
               DESY, 23.--27.~Oct.~2000\stru{0.pt}{4.6mm}}}
      \end{center}
    \end{minipage}%
  \end{turn}    
  \begin{minipage}[t]{\textwidth}
    \stepcounter{chapslide}
    \color{\bpdtcolor}\rule[\footerruledist]{\textwidth}{\footerrulewidth}
    \tiny\footerleft\hfill\footercenter\hfill\footerright
  \end{minipage}%
}


==> LaTeX/examples/talk/ztalk-tit.tex <==
%-------------------------------------------------------------------------------
%       Title page
%-------------------------------------------------------------------------------
{
\begin{boxpage}[e]
%%
%%  title box
%%
{
\putboxparloc{}{1.9pt}{purple}{yellow}{purple}
\putbox{f}{ct}{t}{c}{0}{s}{0}{
  \begin{center}
    \bf\Large
    \stru{2.2ex}{0.ex}
    \LaTeXZ:\kern3.cm\\
    A \LaTeX\ Environment\kern3.cm\\[-3.mm]
    for ZEUS\kern3.cm
    \stru{0.ex}{1.5ex}
  \end{center}}%
}
%%
%%  the LaTeX lion
%%
\putbox{p}{rt}{c}{-20}{20}{350}{380}{figure=plots/lion_yellow.eps,clip=}
%%
%%  name, institute
%%
{
\putboxcolloc{blue}{}{cyan}
\putbox{b}{ct}{t}{c}{700}{s}{0}{
  \begin{center}
     Uli Katz,\\
     University of Bonn
  \end{center}}%
}
%%
%%  the ZEUS logo
%%
\putbox{p}{lt}{c}{80}{1000}{500}{500}{figure=plots/zeus_logo.eps,clip=}
%%
%%  add occasion, date
%%
{
\putboxcolloc{red}{lightyellow}{darkcyan}
\putbox{B}{rt}{c}{-0}{1000}{1070}{400}{
  \begin{center}
     \vfill
     {\large
     Collaboration Meeting}
     \vfill
     DESY, 23-27.~Oct.~2000
     \vfill
  \end{center}}%
}
%%
%%  table of contents
%%
{
\putboxparloc{4.mm}{}{green}{lightestcyan}{black}
\putbox{f}{cb}{c}{c}{-150}{1400}{0}{
    \cbull{\red}{0.7em} {\darkblue Objectives}\\[0.5mm]
    \cbull{\red}{0.7em} {\darkblue Elements}\\[0.5mm]
    \cbull{\red}{0.7em} {\darkblue The bibliography data base}\\[-1.5mm]
           \pbull{1.7em}{\darkgreen\small User interface}\\[-1.5mm]
           \pbull{1.7em}{\darkgreen\small Administration and quality checking}\\
    \cbull{\red}{0.7em} {\darkblue Status and release}
}}
%%
\end{boxpage}
}


==> LaTeX/examples/talk/ztalk-txt.tex <==
\setcounter{chap}{1}
%-------------------------------------------------------------------------------
%       Objectives
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Objectives of \LaTeXZ
  \end{center}}
}
%%
%%  List of main goals of LaTeX4zeus
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{350}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>{\large\magenta Support common ZEUS 
                                         paper style}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Provides well-defined appearence\\[-2.2mm]
                       \>\>(title page layout, fonts, \dots)\\
                       \>\cmin{\green}{-.5em}
                         \>Implementation of rules and conventions\\[-2.2mm]
                       \>\>in {\it The Guide for Writing ZEUS Papers}\\[7.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta Provide user-friendly}\\[-1.mm]
                       \>{\large\magenta \LaTeX\ environment}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Collection of useful \LaTeX\ macros\\
                       \>\cmin{\green}{-.5em}
                         \>Ready-to-use setup for ZEUS drafts,\\[-2.2mm]
                       \>\>preprints, notes, coference contributions\\
                       \>\cmin{\green}{-.5em}
                         \>Easy installation\\
                       \>\cmin{\green}{-.5em}
                         \>Detailed WWW documentation\\[7.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta BiBTeX data base}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Collects all references used by ZEUS\\[-2.2mm]
                       \>\>documents in one central data base.\\
                       \>\cmin{\green}{-.5em}
                         \>High quality standard (new entries\\[-2.2mm]
                       \>\>are checked by scientific editor)\\
                       \>\cmin{\green}{-.5em}
                         \>WWW interface for searching\\[-2.2mm]
                       \>\>and adding entries\\
                       \>\cmin{\green}{-.5em}
                         \>{\darkred Success depends on your 
                                     contributions!}
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Elements
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Elements of \LaTeXZ
  \end{center}}
}
%%
%%  List of main elements of LaTeX4zeus
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{270}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>{\large\magenta Documentation}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>{\green 
                    \texttt{http://giroz.desy.de/ZEUS{\usc}ONLY/LaTeX4zeus}}\\
                       \>\cmin{\green}{-.5em}
                         \>Installation, usage, development \dots\\
                       \>\cmin{\green}{-.5em}
                         \>Message interface\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta Installation mechanism}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>All relevant files in one gzip'ed tar file\\[-2.2mm]
                       \>\>$\Rightarrow$ download, unpack and execute\\[-2.2mm]
                       \>\>\phantom{$\Rightarrow$ }installation script\\
                       \>\cmin{\green}{-.5em}
                         \>Start working ...\\
                       \>\cmin{\green}{-.5em}
                         \>Easy migration for existing projects.\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta \LaTeX\ macros}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Provide all the nice handy utilities\\[-2.2mm]
                       \>\>you always (never?) wanted to have.\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta BiBTeX data base}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Just select your references and use them.\\
                       \>\cmin{\green}{-.5em}
                         \>Provide missing references\\[-2.2mm]
                       \>\>using WWW interface.\\
                       \>\cmin{\green}{-.5em}
                         \>Checking, formatting etc.\ is done for you.\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta An advanced class package for slides}
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Message form
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Message form
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{400}{1800}{0}{figure=plots/l4z_message.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1900}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>Messages are stored in WWW-accessible file\\[2.mm]
  \ \cbull{\red}{-.5em}\>Scientific editor and/or \LaTeXZ\\
                       \>developper will react a.s.a.p.
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Bibliography search form
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Bibliography search form
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{400}{1800}{0}{figure=plots/l4z_search1.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1750}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>You can request a logical {\it and} or {\it or}\\
                       \>of up to 5 search conditions.\\[2.mm]
  \ \cbull{\red}{-.5em}\>Note that search is done in BiBTeX files\\
                       \>containing LaTeX syntax.\\[2.mm]
  \ \cbull{\red}{-.5em}\>Online help available
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Bibliography search results
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Bibliography search results
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{550}{1800}{0}{figure=plots/l4z_search2.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1900}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>You may refine your search by going back\\
                       \>to search form.
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Input form
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Bibliography input form
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{350}{1800}{0}{figure=plots/l4z_input.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1800}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>Mechanism to avoid duplicate identifiers\\[2.mm]
  \ \cbull{\red}{-.5em}\>Mechanism to modify exsting entries\\
                       \>(have to be checked by editor)\\[2.mm]
  \ \cbull{\red}{-.5em}\>Detailed online help\\[2.mm]
  \ \cbull{\red}{-.5em}\>Please adhere to format conventions!
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Life Cycle of a \LaTeXZ BiBTeX entry
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{250}{%
  \begin{center}
  \large\bf Life Cycle of a \LaTeXZ\\[-3.mm]
            BiBTeX entry
  \end{center}}
}
%%
%%  stations
%%
{
\SetWidth{12.0}
\SetColor{Red}
\ArrowLine(450,2150)(450,1650)
\ArrowLine(450,1600)(450,1000)
\ArrowLine(450,1050)(450,350)
}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{350}{900}{0}{%
  \begin{center}
  Entry by user\\
  {\small\darkblue (can be used, preliminary)}
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{850}{900}{0}{%
  \begin{center}
  Entry into\\
  \LaTeXZ data base\\
  {\small\darkblue (fully autorized usage)}
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{1450}{900}{0}{%
  \begin{center}
  Update by user\\
  {\small\darkblue (main entry unchanged, update can be used)}
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{2050}{900}{0}{%
  \begin{center}
  Update in data base\\
  {\small\darkblue (main entry changed, 
  old and temporary versions may remain
  available if necessary)}
  \end{center}
}}
%%
%%  actions
%%
{
\SetWidth{12.0}
\SetColor{Red}
\LongArrow(1000,1900)(500,1900)
\LongArrow(1000,1300)(500,1300)
\LongArrow(1000,700)(500,700)
}
{\putboxparloc{}{1.pt}{darkblue}{lightyellow}{black}
\putbox{f}{rc}{c}{-0}{720}{750}{0}{%
  \begin{center}
  Check by scientific editor\\
  {\small\darkred 
   (reference data,\\ 
   identifier,\\
   \LaTeX\ formatting)

  }
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkblue}{lightyellow}{black}
\putbox{f}{rc}{c}{-0}{1320}{750}{0}{%
  \begin{center}
  Mistake, change,\\
  missing information\\
  detected by user\\
  {\small\darkred 
   (use update mode\\ 
   of \LaTeXZ\\
   input form)

  }
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkblue}{lightyellow}{black}
\putbox{f}{rc}{c}{-0}{1920}{750}{0}{%
  \begin{center}
  Check by scientific editor\\
  {\small\darkred 
   (keep old identifiers\\ 
   connected to\\
   updated data)

  }
  \end{center}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Status and Release
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Status and Release
  \end{center}}
}
%%
%%  Status
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{lt}{c}{0}{300}{1400}{0}{%
  \vspace*{-12.mm}
  \begin{center}{\large\magenta Status:}\end{center}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>First tests successful\\[-2.mm]
                       \>(thanks to Brian Foster, Alex Kappes,\\[-2.mm]
                       \>Matthew Wing for giving it a try)\\[2.mm]
  \ \cbull{\red}{-.5em}\>Meanwhile: lots of improvements\\[-2.mm]
                       \>implemented\\[2.mm]
  \ \cbull{\red}{-.5em}\>Some details have to be finalized.
  \end{tabbing}
}}
%%
%%  Your response
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{lt}{c}{0}{1700}{1400}{0}{%
  \vspace*{-12.mm}
  \begin{center}{\large\magenta Your response:}\end{center}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>{\red Give it a try!}\\[2.mm]
  \ \cbull{\red}{-.5em}\>{\red Please} report problems, criticism,\\[-2.mm]
                       \>suggestions, comments\\[-2.mm]
                       \>(use the message form!)\\[2.mm]
  \ \cbull{\red}{-.5em}\>It is like investing some work now\\[-2.mm]
                       \>to save much more work later\dots
  \end{tabbing}
}}
%%
%%  Release
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{rt}{c}{-0}{1070}{1400}{0}{%
  \vspace*{-12.mm}
  \begin{center}{\large\magenta Release:}\end{center}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>Expected in the next days\\[-2.mm]
                       \>(not later than end of next week)\\[2.mm]
  \ \cbull{\red}{-.5em}\>Will be announced to zeus+all\\[2.mm]
  \ \cbull{\red}{-.5em}\>It's already usable, though! 
  \end{tabbing}
}}
%%
\end{boxpage}


==> LaTeX/zeus/zeus_def.tex <==
%------------------------------------------------------------------------------
%       Standard ZEUS text fragments
%       ----------------------------
%       -> references system footnote
%------------------------------------------------------------------------------
\newcommand{\ZcoosysA}{%
The ZEUS coordinate system is a right-handed Cartesian system, with the $Z$
axis pointing in the proton beam direction, referred to as the ``forward
direction'', and the $X$ axis pointing left towards the center of HERA.
The coordinate origin is at the nominal interaction point.\xspace}
\newcommand{\ZcoosysB}{%
The ZEUS coordinate system is a right-handed Cartesian system, with the $Z$
axis pointing in the proton beam direction, referred to as the ``forward
direction'', and the $X$ axis pointing left towards the centre of HERA.
The coordinate origin is at the nominal interaction point.\xspace}
\newcommand{\Zpsrap}{%
The pseudorapidity is defined as $\eta=-\ln\left(\tan\frac{\theta}{2}\right)$,
where the polar angle, $\theta$, is measured with respect to the proton beam
direction.\xspace}
\newcommand{\ZcoosysfnA}{\footnote{\ZcoosysA}}
\newcommand{\ZcoosysfnB}{\footnote{\ZcoosysB}}
\newcommand{\ZcoosysfnAeta}{\footnote{\ZcoosysA\Zpsrap}}
\newcommand{\ZcoosysfnBeta}{\footnote{\ZcoosysB\Zpsrap}}
%------------------------------------------------------------------------------
%       -> introductory sentence for detector description
%------------------------------------------------------------------------------
\newcommand{\Zdetdesc}{%
A detailed description of the ZEUS detector can be found 
elsewhere~\cite{zeus:1993:bluebook}. A brief outline of the 
components that are most relevant for this analysis is given
below.\xspace}
%------------------------------------------------------------------------------
%       -> CTD description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctddesc}[1]{%
Charged particles were tracked in the central tracking detector (CTD)~\citeCTD,
which operated in a magnetic field of $1.43\Tesla$ provided by a thin 
superconducting coil. The CTD consisted of 72~cylindrical drift chamber 
layers, organized in 9~superlayers covering the polar-angle#1 region 
\mbox{$15^\circ<\theta<164^\circ$}. The transverse-momentum resolution for
full-length tracks is $\sigma(p_T)/p_T=0.0058p_T\oplus0.0065\oplus0.0014/p_T$,
with $p_T$ in $\Gev$.}
%------------------------------------------------------------------------------
%       -> CTD/MVD description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctdmvddesc}[1]{%
In the kinematic range of the analysis, charged particles were tracked
in the central tracking detector (CTD)~\citeCTD, and the microvertex
detector (MVD)~\citeMVD. These components operated in a magnetic
field of $1.43\Tesla$ provided by a thin superconducting solenoid. The
CTD consisted of 72~cylindrical drift chamber layers, organised in
nine superlayers covering the polar-angle#1 region
\mbox{$15^\circ<\theta<164^\circ$}. The MVD consisted of a barrel
(BMVD) and a forward (FMVD) section with three cylindrical layers and
four vertical planes of single-sided silicon strip sensors in the BMVD
and FMVD respectively. The BMVD provided polar-angle coverage for
tracks with three measurements from $30^\circ$ to $150^\circ$. The
FMVD extended the polar-angle coverage in the forward region to
$7^\circ$. After alignment the single hit resolution of the BMVD was
$\rm 25\,\mu m$ and the impact parameter resolution of the CTD-BMVD system
for high momentum tracks was $\rm 100\,\mu m$.}
%------------------------------------------------------------------------------
%       -> CTD/MVD/STT description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctdmvdsttdesc}[1]{%
In the kinematic range of the analysis, charged particles were tracked
in the central tracking detector (CTD)~\citeCTD, the microvertex
detector (MVD)~\citeMVD and the straw-tube tracker (STT)~\citeSTT. The CTD and the MVD
operated in a magnetic field of $1.43\Tesla$ provided by a thin
superconducting solenoid. The CTD drift chamber covered the
polar-angle#1 region \mbox{$15^\circ<\theta<164^\circ$}. The MVD
silicon tracker consisted of a barrel (BMVD) and a forward (FMVD)
section. The BMVD provided polar angle coverage for tracks with three
measurements from $30^\circ$ to $150^\circ$. The FMVD extended the
polar-angle coverage in the forward region to $7^\circ$. The STT
covered the polar-angle region \mbox{$5^\circ<\theta<25^\circ$}.}
%------------------------------------------------------------------------------
%       -> CTD/MVD/STT description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zsttdesc}[1]{%
The STT consisted of 48 sectors of two different sizes. Each sector
contained 192 (small sector) or 264 (large sector) straws of diameter
7.5 mm arranged into 3 layers. The sectors were trapezoidal in shape
and each subtended an azimuthal angle of $60^{\circ}$ -- 6 sectors
formed a so-called superlayer. A particle passing through the complete
detector traversed 8 superlayers, which were rotated around the beam
direction at angles of $30^{\circ}$ or $15^{\circ}$ to each other. The STT
covered the polar-angle region $5^{\circ}<\theta<23^{\circ}$.
}
%------------------------------------------------------------------------------
%       -> CAL description
%------------------------------------------------------------------------------
\newcommand{\Zcaldesc}{%
The high-resolution uranium--scintillator calorimeter (CAL)~\citeCAL consisted 
of three parts: the forward (FCAL), the barrel (BCAL) and the rear (RCAL)
calorimeters. Each part was subdivided transversely into towers and
longitudinally into one electromagnetic section (EMC) and either one (in RCAL)
or two (in BCAL and FCAL) hadronic sections (HAC). The smallest subdivision of
the calorimeter is called a cell.  The CAL energy resolutions, as measured under
test-beam conditions, are $\sigma(E)/E=0.18/\sqrt{E}$ for electrons and
$\sigma(E)/E=0.35/\sqrt{E}$ for hadrons ($E$ in $\Gev$).}
%------------------------------------------------------------------------------
%       -> HES description
%------------------------------------------------------------------------------
\newcommand{\Zhesdesc}{%
The position of electrons scattered at small angles to the
electron-beam directions was determined with the help of RHES\citeHES,
which consisted of a layer of approximately $10\,000$ $(2.96\times
3.32\,{\rm cm^2})$ silicon-pad detectors inserted in the RCAL at a
depth of 3.3 radiation lengths.}
%------------------------------------------------------------------------------
%       -> MUON description
%------------------------------------------------------------------------------
\newcommand{\Zmuondesc}{%
The muon system consisted of rear, barrel (R/BMUON) and forward
(FMUON) tracking detectors. The B/RMUON consisted of limited--streamer
(LS) tube chambers placed behind the BCAL (RCAL), inside and outside a
magnetized iron yoke surrounding the CAL. The barrel and rear muon
chambers cover polar angles from $34^\circ$ to $135^\circ$ and from
$135^\circ$ to $171^\circ$, respectively. The FMUON consisted of six
trigger planes of LS tubes and four planes of drift chambers covering
the angular region from $5^\circ$ to $32^\circ$. The muon system
exploited the magnetic field of the iron yoke and, in the forward
direction, of two iron toroids magnetized to $\approx\,1.6\,{\rm T}$
to provide an independent measurement of the muon momentum.}
%------------------------------------------------------------------------------
%       -> BAC description
%------------------------------------------------------------------------------
\newcommand{\Zbacdesc}{%
The iron yoke surrounding the CAL was instrumented with proportional
drift chambers to form the Backing Calorimeter (BAC)~\citeBAC.  The
BAC consisted of 5142 aluminium chambers inserted into the gaps
between $7.3\,{\rm cm}$ thick iron plates (10, 9 and 7 layers in forecap,
barrel and rearcap, respectively) serving as calorimeter absorber.
The chambers were typically $5\,{\rm m}$ long and had a wire spacing of
$1.5\,{\rm cm}$. The anode wires were covered by $50\,{\rm cm}$ long cathode
pads. The BAC was equipped with energy
readout and position sensitive readout for muon tracking.  The former
was based on 1692 pad towers ($50 \times 50\,{\rm cm^2}$), providing an
energy resolution of $\sim 100\%/\sqrt E$. The position information
from the wires allowed the reconstruction of muon trajectories in two
dimensions ($XY$ in barrel and $YZ$ in endcaps) with spatial accuracy
of a few mm.}
%------------------------------------------------------------------------------
%       -> LUMI description (The actual lumi uncertainty in percent is given as the argument) 
%------------------------------------------------------------------------------
\newcommand{\Zlumidesc}[1]{%
The luminosity was measured using the Bethe--Heitler reaction
$ep\,\rightarrow\, e\gamma p$ by a luminosity detector which consisted
of independent lead-scintillator calorimeter\citePCAL and a magnetic
spectrometer\citeSPECTRO systems. The fractional systematic
uncertainty on the measured luminosity was #1.}
%------------------------------------------------------------------------------
%       -> 6mT description
%------------------------------------------------------------------------------
%\newcommand{\Z6mTdesc}{%
%Scattered electrons emerging from $eP$ interactions at very small
%angles were detected in a small tungsten--scintillator calorimeter
%located approximately 6~m from the interaction point in the rear
%direction, referred to as the ``6m-tagger''~\cite6mT. For
%electrons in the energy range $4.1\le E_e\le7.4$ the acceptance is 
%very close to one with very high purity.}
%------------------------------------------------------------------------------
%       -> Standard Acknowledgements
%------------------------------------------------------------------------------
\newcommand{\Zacknowledge}{%
We appreciate the contributions to the construction and maintenance of the 
ZEUS de- tector of many people who are not listed as authors. The HERA 
machine group and the DESY computing staff are especially acknowledged for 
their success in providing excel- lent operation of the collider and the 
data-analysis environment. We thank the DESY directorate for their strong 
support and encouragement.}
%------------------------------------------------------------------------------
%       Handy macros, mainly for text mode:
%       -----------------------------------
%       -> unknown marker
%------------------------------------------------------------------------------
\newcommand{\xxx}{\hbox{$\qsm\qsm\qsm$}\xspace}
%------------------------------------------------------------------------------
%       -> D0 acronym
%------------------------------------------------------------------------------
\newcommand{\DO}{{D{\O}}\xspace}
%------------------------------------------------------------------------------
%       -> (anti-)something with correct hyphenation
%------------------------------------------------------------------------------
\newcommand{\Anti}[1]{\hbox{(anti-)}\discretionary{}{}{}#1}
\newcommand{\anti}[1]{(anti\discretionary{-)}{}{)}#1}
%------------------------------------------------------------------------------
%       -> characters for typewriter font (used for http addresses)
%------------------------------------------------------------------------------
\chardef\usc=95
\chardef\til=126
%------------------------------------------------------------------------------
%       -> xdotspace (like xspace, but adds period unless
%          another period follows)
%       -> "nn% C.L."
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\DeclareRobustCommand\xdotspace{\futurelet\@let@token\@xdotspace}
\def\@xdotspace{%
  \ifx\@let@token.\else
  \ifx\@let@token\bgroup.\else
  \ifx\@let@token\egroup.\else
  \ifx\@let@token\/.\else
  \ifx\@let@token\ .\else
  \ifx\@let@token~.\else
  \ifx\@let@token!.\else
  \ifx\@let@token,.\else
  \ifx\@let@token:.\else
  \ifx\@let@token;.\else
  \ifx\@let@token?.\else
  \ifx\@let@token/.\else
  \ifx\@let@token'.\else
  \ifx\@let@token).\else
  \ifx\@let@token-.\else
  \ifx\@let@token\@xobeysp.\else
  \ifx\@let@token\space.\else
  \ifx\@let@token\@sptoken.\else
   .\space
   \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}
\catcode`\@=12 % @ signs are no longer letters
\newcommand{\CL}[1]{$#1\%$~C.L\xdotspace}
%------------------------------------------------------------------------------
%       -> vertical rule of width zero and variable height & depth
%------------------------------------------------------------------------------
\newcommand{\stru}[2]{%
   \relax\ifmmode\hbox{\vrule height#1 depth#2 width0pt}%
   \else\vrule height#1 depth#2 width0pt\fi}
%------------------------------------------------------------------------------
%       -> underline with resonable distance text - line
%------------------------------------------------------------------------------
\newcommand{\uline}[1]{$\underline{\hbox{#1\stru{0.pt}{.485ex}}}$}
%------------------------------------------------------------------------------
%       -> roman numbers (uppercase and lowercase)
%------------------------------------------------------------------------------
\newcommand{\Ronum}[1]{\uppercase\expandafter{\romannumeral#1}}
\newcommand{\ronum}[1]{\expandafter{\romannumeral#1}}
%------------------------------------------------------------------------------
%       -> definition for LaTeX4zeus
%------------------------------------------------------------------------------
\DeclareRobustCommand{\LaTeXZ}{%
  \LaTeX\kern-.05em4\kern-.1em
  {\raisebox{-0.2ex}{$\scriptstyle\text{ZEUS}$}}\xspace}
%------------------------------------------------------------------------------
%       -> umlaut definitions for references (needed since BiBTeX 
%          MACRO strings cannot contain quotes)
%------------------------------------------------------------------------------
\newcommand{\Auml}{\"A}
\newcommand{\Ouml}{\"O}
\newcommand{\Uuml}{\"U}
\newcommand{\auml}{\"a}
\newcommand{\ouml}{\"o}
\newcommand{\uuml}{\"u}
%------------------------------------------------------------------------------
%       -> shorthands for equation, figure, table, section references
%          (require standard use of labels: eq-... for equations, cha-...
%           for chapters, sec-... for (sub)sections, tab-... for tables
%           and fig-... for figures)
%------------------------------------------------------------------------------
\newcommand{\eq}[1]{(\ref{eq-#1})}
\newcommand{\eqsand}[2]{(\ref{eq-#1}) and~(\ref{eq-#2})}
\newcommand{\eqsto}[2]{(\ref{eq-#1})--(\ref{eq-#2})}
\newcommand{\eqstwo}[2]{(\ref{eq-#1},\ref{eq-#2})}
\newcommand{\eqsthr}[3]{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3})}
\newcommand{\eqsfou}[4]{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3},\ref{eq-#4})}
\newcommand{\Eq}[1]{Equation~(\ref{eq-#1})}
\newcommand{\Eqsto}[2]{Equations~(\ref{eq-#1})--(\ref{eq-#2})}
\newcommand{\fig}[1]{Fig.~\ref{fig-#1}}
\newcommand{\Fig}[1]{Figure~\ref{fig-#1}}
\newcommand{\figand}[2]{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\newcommand{\Figand}[2]{Figures~\ref{fig-#1} and~\ref{fig-#2}}
\newcommand{\tab}[1]{Table~\ref{tab-#1}}
\newcommand{\Tab}[1]{Table~\ref{tab-#1}}
\newcommand{\taband}[2]{Tables~\ref{tab-#1} and~\ref{tab-#2}}
\newcommand{\cha}[1]{Chap.~\ref{cha-#1}}
\newcommand{\Cha}[1]{Chapter~\ref{cha-#1}}
\newcommand{\sect}[1]{Sect.~\ref{sec-#1}}
\newcommand{\Sect}[1]{Section~\ref{sec-#1}}
\newcommand{\sectand}[2]{Sects.~\ref{sec-#1} and~\ref{sec-#2}}
\newcommand{\sectto}[2]{Sects.~\ref{sec-#1} to~\ref{sec-#2}}
\newcommand{\Sectand}[2]{Sections~\ref{sec-#1} and~\ref{sec-#2}}
\newcommand{\Sectto}[2]{Sections~\ref{sec-#1} to~\ref{sec-#2}}
%------------------------------------------------------------------------------
%       -> log file message
%------------------------------------------------------------------------------
\newcommand{\LogMess}[1]{\typeout{^^J==> #1^^J}}
%------------------------------------------------------------------------------
%       Some special symbols and settings for math mode:
%       ------------------------------------------------
%       -> redefine mathbf
%------------------------------------------------------------------------------
\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{sl}
%------------------------------------------------------------------------------
%       -> physics units (eV and multiples)
%------------------------------------------------------------------------------
\newcommand{\eVdist}{\kern-0.06667em}
\newcommand{\Ev}{{\text{e}\eVdist\text{V\/}}}
\newcommand{\Kev}{{\text{ke}\eVdist\text{V\/}}}
\newcommand{\Mev}{{\text{Me}\eVdist\text{V\/}}}
\newcommand{\Gev}{{\text{Ge}\eVdist\text{V\/}}}
\newcommand{\Tev}{{\text{Te}\eVdist\text{V\/}}}
\newcommand{\ev}{{\,\text{e}\eVdist\text{V\/}}}
\newcommand{\kev}{{\,\text{ke}\eVdist\text{V\/}}}
\newcommand{\mev}{{\,\text{Me}\eVdist\text{V\/}}}
\newcommand{\gev}{{\,\text{Ge}\eVdist\text{V\/}}}
\newcommand{\tev}{{\,\text{Te}\eVdist\text{V\/}}}
%------------------------------------------------------------------------------
%       -> various other units
%------------------------------------------------------------------------------
\newcommand{\mb}{\,\text{mb}}
\newcommand{\mub}{\,\upmu\text{b}}
\newcommand{\nb}{\,\text{nb}}
\newcommand{\pb}{\,\text{pb}}
\newcommand{\fb}{\,\text{fb}}
\newcommand{\mubi}{\,\upmu\text{b}^{-1}}
\newcommand{\mbi}{\,\text{mb}^{-1}}
\newcommand{\nbi}{\,\text{nb}^{-1}}
\newcommand{\pbi}{\,\text{pb}^{-1}}
\newcommand{\fbi}{\,\text{fb}^{-1}}
\newcommand{\met}{\,\text{m}}
% \newcommand{\nm}{\,\text{nm}}
\newcommand{\mum}{\,\upmu\text{m}}
% \newcommand{\mm}{\,\text{mm}}
% \newcommand{\cm}{\,\text{cm}}
\newcommand{\km}{\,\text{km}}
\newcommand{\Amp}{\,\text{A}}
\newcommand{\nA}{\,\text{nA}}
\newcommand{\muA}{\,\upmu\text{A}}
\newcommand{\mA}{\,\text{mA}}
\newcommand{\kA}{\,\text{kA}}
% \newcommand{\Hz}{\,\text{Hz}}
% \newcommand{\kHz}{\,\text{kHz}}
% \newcommand{\MHz}{\,\text{MHz}}
% \newcommand{\GHz}{\,\text{GHz}}
\newcommand{\ppm}{\,\text{ppm}}
\newcommand{\ppb}{\,\text{ppb}}
\newcommand{\scd}{\,\text{s}}
% \newcommand{\ps}{\,\text{ps}}
% \newcommand{\ns}{\,\text{ns}}
\newcommand{\mus}{\,\upmu\text{s}}
\newcommand{\ms}{\,\text{ms}}
% \newcommand{\rad}{\,\text{rad}}
\newcommand{\murad}{\,\upmu\text{rad}}
% \newcommand{\mrad}{\,\text{mrad}}
\newcommand{\gra}{\,\text{g}}
\newcommand{\pg}{\,\text{pg}}
\newcommand{\nang}{\,\text{ng}}
\newcommand{\mug}{\,\upmu\text{g}}
\newcommand{\mg}{\,\text{mg}}
\newcommand{\kg}{\,\text{kg}}
\newcommand{\Tesla}{\,\text{T}}
\newcommand{\Kelvin}{\,\text{K}}
%------------------------------------------------------------------------------
%       -> additional operators
%------------------------------------------------------------------------------
\newcommand{\odiv}{{\operatorname*{div}}}
\newcommand{\ograd}{{\operatorname*{grad}}}
\newcommand{\orot}{{\operatorname*{rot}}}
\newcommand{\odiag}{{\operatorname*{diag}}}
\newcommand{\ocov}{{\operatorname*{cov}}}
%------------------------------------------------------------------------------
%       -> fraction with slash instead of ratio bar
%------------------------------------------------------------------------------
\newcommand{\slashfrac}[2]{%
  \raisebox{0.5ex}{\ensuremath #1}\kern-0.12em/\kern-0.08em
  \raisebox{-.8ex}{\ensuremath #2}}
%------------------------------------------------------------------------------
%       -> shorthand for "integral limits below and above"
%------------------------------------------------------------------------------
\newcommand{\intl}{\int\limits}
\newcommand{\ointl}{\oint\limits}
%------------------------------------------------------------------------------
%       -> d'Alembert operator
%------------------------------------------------------------------------------
\newcommand{\sqr}[3]{%
    {\vcenter{\hrule height.#3ex\hbox{\vrule width.#2ex height#1ex
     \kern#1ex\vrule width.#3ex}\hrule height.#2ex}}}
\newcommand{\dalem}{\mathchoice\sqr{1.3}{08}{24}\sqr{1.4}{08}{24}
                    \sqr{1.15}{07}{21}\sqr{1.0}{06}{18}\,}
%------------------------------------------------------------------------------
%       -> vectors and matrices
%------------------------------------------------------------------------------
\newcommand{\vect}[1]{\begin{matrix}#1\end{matrix}}
\newcommand{\pvect}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\bvect}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\vvect}[1]{\begin{vmatrix}#1\end{vmatrix}}
\newcommand{\Vvect}[1]{\begin{Vmatrix}#1\end{Vmatrix}}
%------------------------------------------------------------------------------
%       -> antiparticles and particles with a bar in parentheses
%------------------------------------------------------------------------------
\newcommand{\widebar}[1]{%
   \mkern1.5mu\overline{\mkern-1.5mu#1\mkern-1.mu}\mkern1.mu}
\catcode`\@=11 % @ signs are now treated as letters
\newcommand{\parenbar}{\mathpalette\p@renb@r}
\def\p@renb@r#1#2{\vbox{%
  \ifx#1\scriptscriptstyle \dimen@.7em\dimen@ii.2em\else
  \ifx#1\scriptstyle \dimen@.8em\dimen@ii.25em\else
  \dimen@1em\dimen@ii.4em\fi\fi \offinterlineskip
  \ialign{\hfill##\hfill\cr
    \vbox{\hrule width\dimen@ii}\cr
    \noalign{\vskip-.3ex}%
    \hbox to\dimen@{$\mathchar300\hfil\mathchar301$}\cr
    \noalign{\vskip-.3ex}%
    $#1#2$\cr}}}
\catcode`\@=12 % @ signs are no longer letters
\newcommand{\nuan}{\parenbar{\nu}}
\newcommand{\nunubar}{\parenbar{\nu}}
\newcommand{\ppbar}{\parenbar{p}}
\newcommand{\qqbar}{\parenbar{q}}
\newcommand{\pbar}{\widebar{p}}
\newcommand{\nbar}{\widebar{n}}
\newcommand{\qbar}{\widebar{q}}
\newcommand{\dbar}{\widebar{d}}
\newcommand{\ubar}{\widebar{u}}
\newcommand{\sbar}{\widebar{s}}
\newcommand{\cbar}{\widebar{c}}
% \newcommand{\bbar}{\widebar{b}}
\newcommand{\tbar}{\widebar{t}}
\newcommand{\nubar}{\widebar{\nu}}
\newcommand{\Dbar}{\widebar{D}}
\newcommand{\ebar}{\widebar{e}}
\newcommand{\Ebar}{\widebar{e}}
\newcommand{\Hebar}{\widebar{\text{He}}}
\newcommand{\Cbar}{\widebar{\text{C}}}
\newcommand{\Abar}{\widebar{\text{A}}}
\newcommand{\Kbar}{\widebar{K}}
\newcommand{\chibar}{\widebar{\chi}}
\newcommand{\LQbar}{\widebar{\rm LQ}}
%------------------------------------------------------------------------------
%       -> small numbers
%------------------------------------------------------------------------------
\newcommand{\zero}{{\scriptscriptstyle 0}}
\newcommand{\sone}{{\scriptscriptstyle 1}}
\newcommand{\stwo}{{\scriptscriptstyle 2}}
\newcommand{\sthr}{{\scriptscriptstyle 3}}
\newcommand{\sfou}{{\scriptscriptstyle 4}}
\newcommand{\sfiv}{{\scriptscriptstyle 5}}
\newcommand{\ssix}{{\scriptscriptstyle 6}}
\newcommand{\ssev}{{\scriptscriptstyle 7}}
\newcommand{\seig}{{\scriptscriptstyle 8}}
\newcommand{\snin}{{\scriptscriptstyle 9}}
\newcommand{\sten}{{\scriptscriptstyle 10}}
\newcommand{\half}{{\scriptscriptstyle 1/2}}
%------------------------------------------------------------------------------
%       -> abbreviations for common math mode symbols
%------------------------------------------------------------------------------
\newcommand{\MSbar}{\hbox{$\overline{\rm MS}$}\xspace}
\newcommand{\UO}{{\rm U}(1)_\sY}
\newcommand{\SUT}{{\rm SU}(2)_\sL}
\newcommand{\SUTH}{{\rm SU}(3)_c}
\newcommand{\SUTUO}{{\rm SU}(2)_\sL\times{\rm U}(1)_\sY}
\newcommand{\SUTSUTUO}{{\rm SU}(3)_c\times{\rm SU}(2)_\sL\times{\rm U}(1)_\sY}
\newcommand{\alsmu}[1]{{\alpha_s(\mu_{#1}^2)}}
\newcommand{\alsmz}{{\alpha_s(M_Z^2)}}
\newcommand{\alsqs}{{\alpha_s(Q^2)}}
\newcommand{\als}{\alpha_s}
\newcommand{\ctwb}{\cos\theta_W}
\newcommand{\ctws}{\cos^2\theta_W}
\newcommand{\diff}{{\rm d}}
\newcommand{\gh}{{\gamma_h}}
\newcommand{\lsq}[1]{{\lambda_{#1}}}
\newcommand{\lsqp}[1]{{\lambda'_{#1}}}
\newcommand{\lsqpp}[1]{{{\lambda''}_{#1}}}
\newcommand{\rnge}{\hbox{$\,\text{--}\,$}}
\newcommand{\sihat}{{\hat\sigma}}
\newcommand{\sitil}{{\tilde\sigma}}
\newcommand{\stwb}{\sin\theta_W}
\newcommand{\stwss}{\sin^4\theta_W}
\newcommand{\stws}{\sin^2\theta_W}
\newcommand{\ta}{{\theta^\ast}}
\newcommand{\tilR}{\tilde R}
\newcommand{\tilS}{\tilde S}
\newcommand{\tilU}{\tilde U}
\newcommand{\tilV}{\tilde V}
\newcommand{\tl}{{\theta_\ell}}
\newcommand{\tw}{\theta_W}
%------------------------------------------------------------------------------
%       -> roman character combinations to be used in math mode, mainly
%          sub- or superscripts
%------------------------------------------------------------------------------
\newcommand{\Born}{{\rm Born}}
\newcommand{\BR}{{\rm BR}}
\newcommand{\CC}{{\rm CC}}
\newcommand{\CI}{{\rm CI}}
\newcommand{\CJ}{{\rm CJ}}
\newcommand{\DA}{{\rm DA}}
\newcommand{\DCA}{{\rm DCA}}
\newcommand{\GRV}{{\rm GRV}}
\newcommand{\IC}{{\rm IC}}
\newcommand{\ISR}{{\rm ISR}}
\newcommand{\IP}{{\rm I$\kern-0.01667em$P}\xspace}
\newcommand{\JB}{{\rm JB}}
\newcommand{\LL}{{\rm LL}}
\newcommand{\LQ}{{\rm LQ}}
\newcommand{\LR}{{\rm LR}}
\newcommand{\MC}{{\rm MC}}
\newcommand{\NC}{{\rm NC}}
\newcommand{\NS}{{\rm NS}}
\newcommand{\QPM}{{\rm QPM}}
\newcommand{\RL}{{\rm RL}}
\newcommand{\RPv}{{{\not R}_P}}
\newcommand{\RR}{{\rm RR}}
\newcommand{\SM}{{\rm SM}}
\newcommand{\bkg}{{\rm bkg}}
\newcommand{\cut}{{\rm cut}}
\newcommand{\data}{{\rm data}}
\newcommand{\sdet}{{\rm det}}
\newcommand{\dof}{{\rm dof}}
\newcommand{\eff}{{\rm eff}}
\newcommand{\elm}{{\rm elm}}
\newcommand{\evt}{{\rm evt}}
\newcommand{\exc}{{\rm exc}}
\newcommand{\fit}{{\rm fit}}
\newcommand{\had}{{\rm had}}
\newcommand{\jet}{{\rm jet}}
\newcommand{\meas}{{\rm meas}}
\newcommand{\miss}{{\rm miss}}
\newcommand{\obs}{{\rm obs}}
\newcommand{\pnt}{{\rm pnt}}
\newcommand{\sL}{{\rm L}}
\newcommand{\sR}{{\rm R}}
\newcommand{\sS}{{\rm S}}
\newcommand{\sT}{{\rm T}}
\newcommand{\sY}{{\rm Y}}
\newcommand{\sca}{{\rm sca}}
\newcommand{\sexp}{{\rm exp}}
\newcommand{\sint}{{\rm int}}
\newcommand{\smin}{{\rm min}}
\newcommand{\smax}{{\rm max}}
\newcommand{\srad}{{\rm rad}}
\newcommand{\sthe}{{\rm the}}
\newcommand{\sys}{{\rm sys}}
\newcommand{\tot}{{\rm tot}}
\newcommand{\true}{{\rm true}}
%------------------------------------------------------------------------------
%       -> some calligraphic symbols and applications
%------------------------------------------------------------------------------
\newcommand{\Cor}{{\cal C}}
\newcommand{\F}{{\cal F}}
\newcommand{\Lumi}{{\cal L}}
\newcommand{\Prob}{{\cal P}}
\newcommand{\ord}[1]{{\cal O}(#1)}
\newcommand{\ordlr}[1]{{\cal O}\left(#1\right)}
%------------------------------------------------------------------------------
%       -> some math symbols (+,-,...) for usage as mathchar's
%------------------------------------------------------------------------------
\mathchardef\qsm=63
\mathchardef\pls=43
\mathchardef\mns=512
\mathchardef\plm=518
\mathchardef\eql=61
\mathchardef\smallleft=300
\mathchardef\smallright=301
\mathchardef\les=316
\mathchardef\gre=318
\mathchardef\leq=532
\mathchardef\grq=533
%------------------------------------------------------------------------------
%       Additional functionality for tables and figures
%       -----------------------------------------------
%       -> alignment tools for tables
%------------------------------------------------------------------------------
\newcommand{\cA}{{\phantom{0}}}
\newcommand{\cB}{{\phantom{00}}}
\newcommand{\cC}{{\phantom{000}}}
\newcommand{\cD}{{\phantom{0000}}}
\newcommand{\cAp}{{\phantom{0.}}}
\newcommand{\cM}{{\phantom{\mns}}}
\newcommand{\cP}{{\phantom{\pls}}}
%------------------------------------------------------------------------------
%       -> comments on figures (allow to add axodraw and picture items)
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newcounter{pict@width}
\newcounter{pict@height}
\newlength{\pict@scale}
\setlength{\pict@scale}{0.1mm}
\newcommand{\psfigadd}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox to #2{\hspace{-\fill}\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcounter{pict@widthfst}
\newcounter{pict@widthscd}
\newcounter{pict@widthtot}
\newcommand{\psfigaddtwo}[7]{%
\setcounter{pict@widthfst}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthscd}{1*\ratio{#2+#4+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthtot}{1*\ratio{#2+#4+#6+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\hspace{-\fill}\begin{picture}(\thepict@widthtot,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\put(\thepict@widthscd,0){\psfig{figure=#5,width=#6,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#7}
\end{picture}}
}
\newcommand{\psfigror}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,\thepict@height){\psfig{figure=#1,width=#3,height=#2,clip=,angle=270}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcommand{\psfigrol}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#3,height=#2,clip=,angle=90}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\catcode`\@=12 % @ signs are no longer letters
%------------------------------------------------------------------------------
%       -> narrow figures in list environment
%------------------------------------------------------------------------------
\newlength\listtextwidth
\newcommand{\shiftfloat}[1]{
  \setlength{\listtextwidth}{\textwidth}
  \addtolength{\listtextwidth}{-#1}}
%------------------------------------------------------------------------------
%       -> "none" marker
%------------------------------------------------------------------------------
\newcommand{\none}{\hbox{---}}
%------------------------------------------------------------------------------
%       -> protected commands in captions
%------------------------------------------------------------------------------
\newcommand{\pcite}[1]{{\protect\cite{#1}}}
\newcommand{\pnl}{\protect{\newline}}
%------------------------------------------------------------------------------
%       -> pseudo-footnotes for tables
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newlength{\@tabfninsert}
\newlength{\@tabfnwidth}
\newcommand{\tabfootnote}[2]{%
  \setlength{\@tabfninsert}{0.8em}
  \setlength{\@tabfnwidth}{\textwidth}
  \addtolength{\@tabfnwidth}{-\@tabfninsert}
  \addtolength{\@tabfnwidth}{-0.4em}
  \noindent\makebox[\@tabfninsert][r]{\footnotesize$^{#1}$\hfil}\hfill%
  \parbox[t]{\@tabfnwidth}{\footnotesize #2\hfill}}
\catcode`\@=12 % @ signs are no longer letters

